Learning Methods for Dynamic Topic Modeling in Automated Behaviour Analysis

Semi-supervised and unsupervised systems provide operators with invaluable support and can tremendously reduce the operators load. In the light of the necessity to process large volumes of video data and provide autonomous decisions, this work proposes new learning algorithms for activity analysis in video. The activities and behaviours are described by a dynamic topic model. Two novel learning algorithms based on the expectation maximisation approach and variational Bayes inference are proposed. Theoretical derivations of the posterior of model parameters are given. The designed learning algorithms are compared with the Gibbs sampling inference scheme introduced earlier in the literature. A detailed comparison of the learning algorithms is presented on real video data. We also propose an anomaly localisation procedure, elegantly embedded in the topic modeling framework. The proposed framework can be applied to a number of areas, including transportation systems, security and surveillance.

==> TNNLS-2016-P-6800-R1-Danil_bio.tex <==
{Danil Kuzin}
is a PhD student at the Department of Automatic Control and Systems Engineering at the University of Sheffield and an engineer at the Rinicom, Ltd. He received the Specialist degree in Applied Mathematics and Computer Science, 2012, from Lomonosov Moscow State University, Moscow, Russia. His research is mainly in sparse modelling for video. His other research interests include nonparametric Bayes and deep reinforcement learning.

==> TNNLS-2016-P-6800-R1-Mila_bio.tex <==
{Lyudmila Mihaylova} (M'98,
SM'2008) is Professor of Signal Processing and Control at the
Department of Automatic Control and Systems Engineering at the
University of Sheffield, United Kingdom. Her research is in the
areas of machine learning and autonomous systems with various
applications such as navigation, surveillance and sensor network
systems. She has given a number of talks and tutorials, including
the plenary talk for the IEEE Sensor Data Fusion 2015 (Germany),
invited talks University of California, Los Angeles, IPAMI Traffic
Workshop 2016 (USA), IET ICWMMN 2013 in Beijing, China. Prof.
Mihaylova is an Associate Editor of the IEEE Transactions on
Aerospace and Electronic Systems and of the Elsevier Signal
Processing Journal. She was elected in March 2016 as a president of
the International Society of Information Fusion (ISIF). She is on
the board of Directors of ISIF and a Senior IEEE member. She was the
general co-chair IET Data Fusion $\&$ Target Tracking 2014 and 2012
Conferences, Program co-chair for the 19th International Conference
on Information Fusion, 2016, academic chair of
Fusion 2010 conference.

==> TNNLS-2016-P-6800-R1-Olga_bio.tex <==
{Olga Isupova}
is a PhD student at the Department of Automatic Control and Systems Engineering at the University of Sheffield and an Early Stage Researcher in the FP7 Programme TRAX. She received the Specialist (eq. to M.Sc.) degree in Applied Mathematics and Computer Science, 2012, from Lomonosov Moscow State University, Moscow, Russia. Her research is on machine learning, Bayesian nonparametrics, anomaly detection. 
